Low-Fidelity End-to-End Video Encoder Pre-training for Temporal Action Localization

Temporal action localization (TAL) is a fundamental yet challenging task in video understanding. Existing TAL methods rely on pre-training a video encoder through action classification supervision. This results in a task discrepancy problem for the video encoder -- trained for action classification, but used for TAL. Intuitively, end-to-end model optimization is a good solution. However, this is not operable for TAL subject to the GPU memory constraints, due to the prohibitive computational cost in processing long untrimmed videos. In this paper, we resolve this challenge by introducing a novel low-fidelity end-to-end (LoFi) video encoder pre-training method. Instead of always using the full training configurations for TAL learning, we propose to reduce the mini-batch composition in terms of temporal, spatial or spatio-temporal resolution so that end-to-end optimization for the video encoder becomes operable under the memory conditions of a mid-range hardware budget. Crucially, this enables the gradient to flow backward through the video encoder from a TAL loss supervision, favourably solving the task discrepancy problem and providing more effective feature representations. Extensive experiments show that the proposed LoFi pre-training approach can significantly enhance the performance of existing TAL methods. Encouragingly, even with a lightweight ResNet18 based video encoder in a single RGB stream, our method surpasses two-stream ResNet50 based alternatives with expensive optical flow, often by a good margin.

==> sections/0-abstract.tex <==
Temporal action localization (TAL) is a fundamental yet challenging task in video understanding. Existing TAL methods rely on pre-training a video encoder through action classification supervision.
%
This results in a task discrepancy problem for the video encoder -- trained for action classification, but used for TAL.
%
Intuitively, end-to-end model optimization is a good solution.
%
However, this is not operable for TAL subject to the GPU memory constraints, due to the prohibitive computational cost in processing long untrimmed videos.
%
In this paper we resolve this challenge by
introducing a novel low-fidelity end-to-end (\lofi{}) video encoder pre-training method.
%
Instead of always using the full training configurations
for TAL learning,
we propose to reduce the mini-batch composition in terms of 
temporal, spatial or spatio-temporal resolution
so that end-to-end optimization for the video encoder 
becomes operable under the memory conditions of
a mid-range hardware budget. 
%
Crucially, this enables the gradient to flow backwards through the video encoder from a TAL loss supervision, favourably solving the task discrepancy problem and providing more effective feature representations.
%
Extensive experiments show that the proposed \lofi{} pre-training approach
can significantly enhance the performance of existing TAL methods. 
% \BM{[What bout this to close the abstract?:] 
% Encouragingly, we achieve state-of-the-art performance despite using a single-stream TSM-ResNet18 as the video encoder, surpassing two-stream ResNet50-based alternatives.
% }
Encouragingly, even with a lightweight ResNet18 based video encoder in a single RGB stream, our method surpasses two-stream ResNet50 based alternatives with expensive optical flow, often by a good margin.


==> sections/1-introduction.tex <==
\section{Introduction}
% \begin{figure}
%     \centering
%     \includegraphics[trim={6.5cm 0cm 6.5cm 0cm}, width=0.45\textwidth,clip] {figs/LoFiTAL_Intro.pdf}
%     \caption{
%     A typical temporal action localization (TAL) model is composed of a video encoder and a TAL head.
%     For model optimization two stages are often involved:
%     (1) pre-training the video encoder on a large video classification dataset 
%     %\BM{[isn't this confusing at this point?] (and optionally on a clip version of the target dataset)} 
%     with action classification task's supervision (\textbf{\em top-left circle}),
%     and 
%     (2) training the TAL head on the target action localization dataset (\textbf{\em top-right circle}) whilst freezing the video encoder.
%     %
%     This standard training method
%     leads to a task discrepancy issue with the video encoder --
%     trained for video classification but used for TAL.
%     %
%     To overcome this limitation, 
%     we introduce an extra stage in-between that optimizes
%     both the video encoder and the TAL head
%     end-to-end at a low temporal and/or spatial resolution (\ie, low-fidelity) subject to the same GPU memory constraints (\textbf{\em bottom-middle circle}).
%     % 
%     %Why no {\em end-to-end optimization} of video encoder and TAL head, which could improve the entire model potentially?
%     % This is because with long untrimmed videos as training samples in TAL, end-to-end training is hardly affordable
%     % in practice due to the memory constraint of GPUs.
%     % Intuitively, overcoming this obstacle is beneficial.
%     % With a systematic investigation, in this work we present a low-fidelity end-to-end training strategy.
%     }
%     \label{fig:train_pipepline}
% \end{figure}



Video analysis has recently become an increasingly important area of research, encompassing multiple relevant problems such as action recognition \cite{carreira2017quo,feichtenhofer2016convolutional}, temporal action localization~\cite{zhao2019hacs,CabaHeilbron2016,Escorcia2016DAPsDA,caba2015activitynet,xu2020boundary,xu2020g,Gao_Shi_Wang_Li_Yuan_Ge_Zhou_2020}, and video question answering \cite{huang2020aligned,lei2018tvqa}. % among others.
%
Among those, temporal action localization (TAL) 
\cite{zhao2019hacs,caba2015activitynet} is a fundamental yet challenging task, as natural %in-the-wild 
videos are not temporally trimmed.
%
Given an untrimmed video, TAL aims to identify the start and end points of all action instances and recognize their category labels simultaneously.
%
A typical TAL pipeline is based on deep CNNs composed of two modules: 
a video encoder and a TAL head.
The video encoders are often shared across different TAL pipelines (\eg, G-TAD~\cite{xu2020g}, BC-GNN~\cite{Bai2020bcgnn}), 
by taking a specific off-the-shelf action classification model (\eg, C3D~\cite{7410867}, I3D~\cite{carreira2017quo}, TSM~\cite{lin2019tsm}), with differences only in the TAL head.
%
Instead of short (\eg, 10 seconds) trimmed video clips as in action recognition, 
TAL's input videos are characterized by
much longer temporal duration and bigger data volume, \ie, raw videos without any manual trimming.
%
This causes unique computational challenges that remain
unsolved particularly in model optimization.




In standard optimization of a TAL model,
two stages are often involved:
\begin{enumerate}
    \item First, pre-training the video encoder on a large source video classification dataset (\eg, Kinetics \cite{zisserman2017kinetics})
    and optionally on the clip version of the target dataset
    under {\em action classification supervision};
    \item Second, training the TAL head on the target action localization dataset (\eg, ActivityNet \cite{caba2015activitynet}) under 
    {\em TAL task supervision}, whilst freezing the video encoder's parameters.
\end{enumerate}

With this standard training method, however, the video encoder is only optimal for action classification but not for the target TAL task.
Trained to be invariant to all the short segments of an action instance (as designed in the first stage), the video encoder has inferior sensitivity to 
action temporal boundaries which a TAL model aims to detect.
We call this \textbf{\em a task discrepancy problem}.
%
Consequently, the final TAL model could suffer from suboptimal performance since feature representation 
generally plays a critical role in deep learning.

% model generalization \cite{?}.

% This results in both domain drift and lack of sensitivity to temporal boundaries -- action recognition forces the predictions to be the same across all segments of the video. In order to partially bridge this gap, some methods have resorted to some sort of pre-training on the target data, usually relying on a proxy task that does not necessarily correlate with the final task of temporal action localization [cite, cite].

% {\bf (1)} pre-training the video encoder on a large video class dataset (\eg, Kinetics \cite{zisserman2017kinetics}) with video classification supervision,
% and then
% {\bf (2)} training the localization head on the target action localization dataset (\eg, ActivityNet \cite{caba2015activitynet}) with temporal action localization supervision, whilst freezing the video encoder's parameters.

Intuitively, {\em end-to-end optimization} of video encoder and TAL head could simply solve the above limitation with the standard supervised training method.
Unfortunately, it is not that straightforward for TAL model optimization. 
As mentioned above, model training is severely restricted
by the large input size of untrimmed videos and
subject to the memory constraint of GPUs.
This is why the two-step training method as described above 
becomes the most common and feasible choice during optimizing a TAL model in practice.
Regardless, we believe that solving this limitation of the TAL training design bears a great potential for improving model performance. 

In this work, we present a simple yet effective 
{\em low-fidelity end-to-end} (\lofi{}) 
video encoder pre-training method
particularly designed for better TAL model optimization.
This eliminates the above task discrepancy issue (video classification vs. TAL) from video encoder pre-training.
This is achieved by introducing 
% \BM{[What about:] a surprisingly simple strategy consisting on...} 
a surprisingly simple strategy characterized with
a novel stage of optimizing
both the video encoder and the TAL head
end-to-end using a lower temporal and/or spatial resolution
(\ie, low-fidelity) in the mini-batch construction.
%
As compared to the standard training method, our proposed training strategy does not increase the GPU memory standard
(often a hard constraint for many practitioners).
%
% which is often a hard constraint for many practitioners in practice.
%
Crucially, with our \lofi{} training
% we train the down-scaled temporal action localization model, 
the gradients back-propagate to the video encoder from a temporal action localization loss whilst conditioned on the target TAL head, enabling the learning of video encoder sensitive to the temporal localization objective. 

We make the following {\bf contributions} in this work.
{\bf (1)}
We investigate the limitations of the standard optimization method for TAL models, and consider that 
the task discrepancy problem with the video encoder
would harm the performance of existing TAL models.
This is caused by complex/heavy model design and GPU memory constraints jointly.
Despite a potentially significant ingredient,
video encoder optimization is largely ignored by existing TAL methods without systematic investigation.
%
{\bf (2)}
To improve TAL model optimization, we present a novel, simple, and effective {\em low-fidelity end-to-end} (\lofi{}) video encoder pre-training method.
{\bf (3)}
Extensive experiments show that the proposed \lofi{} yields a new state-of-the-art performance when combined with 
off-the-shelf TAL models (\eg, G-TAD \cite{xu2020g})
despite using a lightweight ResNet18-based video encoder and
merely RGB video frames without the need of computationally expensive
optical flow, thus also enjoying far superior inference efficiency.
% without architectural additions and changes
% on two standard temporal action localization benchmarks. 
%
% integrated into is superior to the existing action classification-based pre-training counterpart, and achieves new state-of-the-art performance.
%
% In summary, the main contributions of our work are: I) to re-think the training strategy for temporal action localization, bringing it towards standard end-to-end training, the overwhelmingly dominant approach in the field II) Propose and empirically evaluate several trade-offs III) Thoroughly evaluate our method, showing the superior performance of our approach to other methods.
%
% Extensive experiments show that the proposed [name] is superior to the existing action classification-based pre-training counterpart, and achieves new state-of-the-art performance.
%
% , which could improve the entire model potentially?
% This is because with long untrimmed videos as training samples in TAL, end-to-end training is hardly affordable
% in practice due to the memory constraint of GPUs.
% Intuitively, overcoming this obstacle is beneficial.
%
% However, the rapid increase on the data input size results in a wide range of computational challenges %that are hard to address 
% in practice, and bars the direct application of image-based know how.  




% The use of unsegmented videos exacerbate the aforementioned computational challenges, to the point that most existing methods (including state-of-the-art ones) heavily rely on feature extractors trained on action classification tasks [cite, cite]. This results in both domain drift and lack of sensitivity to temporal boundaries -- action recognition forces the predictions to be the same across all segments of the video. In order to partially bridge this gap, some methods have resorted to some sort of pre-training on the target data, usually relying on a proxy task that does not necessarily correlate with the final task of temporal action localization [cite, cite].

% In this paper we pre-training on the target dataset. But instead of sacrificing the target task for more tractable a proxy task (e.g. classification), we sacrifice instead temporal and/or spatial resolution of the input and maintain target task. When we train the down-scaled temporal action localization model, the gradient flow back-propagates to the video encoders from a temporal action localization loss, which enables the learning of video encoders sensitive to the temporal localization task. Extensive experiments show that the proposed [name] is superior to the existing action classification-based pre-training counterpart, and achieves new state-of-the-art performance. 

% Given the nature of this e2e learning, we may sell it in perspective of evaluating e2e particularly for TAL. We may first want to highlight the challenge of model training in TAL, and carefully review the development of TAL in terms of model training. Now the most common practice is pretraining video encoder and then frozen it to train the TAL model. E2e training of video encoder and TAL is often not consider. Why? This is due to memory limitation especially in early days. However, this restriction is now gradually relieved but e2e training is kind of forgotten. 

% In summary, the main contributions of our work are: I) to re-think the training strategy for temporal action localization, bringing it towards standard end-to-end training, the overwhelmingly dominant approach in the field II) Propose and empirically evaluate several trade-offs III) Thoroughly evaluate our method, showing the superior performance of our approach to other methods.

% Extensive experiments show that the proposed [name] is superior to the existing action classification-based pre-training counterpart, and achieves new state-of-the-art performance.


==> sections/5-conclusion.tex <==

\section{Conclusion}
In this work we have presented a simple and effective low-fidelity end-to-end (\lofi{}) video encoder pre-training method
for achieving more effective TAL models. 
This is motivated by an observation that in existing TAL methods
the video encoder is merely pre-trained by action classification supervision on short video clips, lacking desired optimization {\wrt} the target temporal localization supervision.
%
Indeed, end-to-end model optimization itself is not novel. 
However, this is non-trivial to conduct for training a TAL model, due to large per-video size that would easily overwhelm the GPU memory, rendering it infeasible in practice.
%
To overcome this obstacle, we propose to reduce the mini-batch construction configurations in the temporal and spatial dimensions of training videos so that end-to-end optimization becomes operable 
under the same memory condition.
%
%We evaluated extensively the LF-E2E method
Extensive experiments demonstrate that our method can clearly improve the performance of existing off-the-shelf TAL models, yielding new state-of-the-art performance even with only RGB modality as input and a more lightweight backbone based single-stream video encoder
on two representative TAL benchmarks.
Further, in-depth ablation studies have also been conducted to break down
the performance benefits from different training steps and mini-batch configurations.

